The history of LHCb

In this paper we describe the history of the LHCb experiment over the last three decades, and its remarkable successes and achievements. LHCb was conceived primarily as a b-physics experiment, dedicated to CP violation studies and measurements of very rare b decays, however the tremendous potential for c-physics was also clear. At first data taking, the versatility of the experiment as a general-purpose detector in the forward region also became evident, with measurements achievable such as electroweak physics, jets and new particle searches in open states. These were facilitated by the excellent capability of the detector to identify muons and to reconstruct decay vertices close to the primary pp interaction region. By the end of the LHC Run 2 in 2018, before the accelerator paused for its second long shut down, LHCb had measured the CKM quark mixing matrix elements and CP violation parameters to world-leading precision in the heavy-quark systems. The experiment had also measured many rare decays of b and c quark mesons and baryons to below their Standard Model expectations, some down to branching ratios of order 10-9. In addition, world knowledge of b and c spectroscopy had improved significantly through discoveries of many new resonances already anticipated in the quark model, and also adding new exotic four and five quark states.

==> Chapter_2_detector_old.tex <==

\subsection{Overview}
\label{sez:detector}

The LHCb~\cite{lhcb_}detector  is a forward spectrometer (figure~\ref{fig:lhcb_dect})
installed at Intersection Point 8 of the LHC,  in the cavern used by the DELPHI experiment during the LEP era. 
A modification to the LHC optics,  shifting the  interaction point
by about 11~m from the centre, allowed maximum use of the cavern space. In this way the detector
length is about 20~m and the total dimensions are about $6 \times 5 \times 20 \ \hbox{m}^{3}$.\\
The angular acceptance goes from approximately 
10~mrad to 300~mrad (figure~\ref{fig:bending}) in the horizontal bending plane,  and 
from 10~mrad to 250~mrad in the vertical  plane 
(figure~\ref{fig:lhcb_dect}). With such acceptance the detector is able to reconstruct
about 20\% of all $b \bar b$ produced.

To measure the momentum of charged particles a dipole magnet producing a vertical magnetic field is used. 
It is a warm magnet  with saddle-shaped coils in a window-frame yoke with sloping poles in
order to match the required detector acceptance, providing an integrated field of 4 Tm. The 
design of the magnet allows to have a fringe 
field level inside the RICHs envelope less than 2mT and a field as high as possible in the regions between
the  tracking stations.

The tracking system~\cite{track} consists of a vertex locator system  (VELO)~\cite{velo},
located around the interaction region, and four planar tracking stations: the TT tracker,
upstream of the dipole magnet, and three tracking stations T1-T3 downstream of the magnet.\\
T1-T3 stations consist of an Inner Tracker (IT), located at the center of the stations and
close to the beam pipe, and of an Outer Tracker (OT) for the outer parts: a minimum momentum of 1.5~GeV/$c$ is
needed to reach the tracking stations \cite{LHCbPerf}.\\

\begin{figure}[!htbp]
\begin{center}
\includegraphics[height=7cm]{figures/lhcb_dect.pdf}
\end{center}
\caption{The LHCb detector: side view}\label{fig:sideview}
\end{figure}
\begin{figure}[!htbp]
\begin{center}
\includegraphics[height=7cm]{figures/bending.pdf}
\end{center}
\caption{The LHCb detector: top view}\label{fig:topview}
\end{figure}
\newpage

Particle identification is a fundamental characteristic of LHCb. 
It is essential for the goals of
the experiment to separate pions from kaons produced in decays. Accurate  reconstruction of electrons, photons and muons
is crucial for flavour tagging. All these tasks are accomplished by a set of specialized detectors.  

 At large polar angles the
momentum spectrum is softer while at small polar angles the momentum spectrum is harder; hence
the particle identification system consists of two RICH detectors to cover the full momentum
range. The upstream detector, RICH 1, covers the low momentum charged particle range 
$\simeq 1–60$ GeV/c using aerogel and $\hbox{C}_{4}\hbox{F}_{10}$  radiators, 
while the downstream detector, RICH 2, covers the
high momentum range from 15 GeV/c up to and beyond 100 GeV/c using a $\hbox{C}\hbox{F}_{4}$ radiator (see
figure zz). RICH 1 has a wide acceptance covering the full LHCb acceptance from $\pm 25$ mrad to
$\pm 300$ mrad (horizontal) and $\pm 250$ mrad (vertical) and is located upstream of the magnet to detect
the low momentum particles. RICH 2 is located downstream of the magnet and has a limited
angular acceptance of  $\pm15$ mrad to  $\pm 120$ mrad (horizontal) and $\pm 100 mrad$ (vertical) but covers
the region where high momentum particles are produced. 

Two calorimeters, one electromagnetic (ECAL) and another hadronic (HCAL), supplemented by a 
Preshower Detector (SPD/PS) \cite{cal},  provide identification of electrons, photons and hadrons
and measurement of their energy. The latter quantity is used at the trigger level to select candidates on the basis of their
transverse energy. Muons play a crucial role in the majority of measurements because of the cleanliness oif thei 
signature. Their identification is provided by five stations (M1 --  M5) interspersed with iron filters. The Muon
Detector also supplies the muon transverse momentum to the trigger. 
i
The different stages will be briefly described in the foillowing.


\subsection{Vertex Locator}

The Vertex Locator( VELO)  is used to reconstruct the production and decay vertex of $b$ and $c$ hadrons,
to provide accurate measurements of their mean life and to measure the impact parameter of
the various tracks related to the PV. It is able to detect particles with pseudorapidity in the range
$1.6~<~\eta~<~4.9$ and coming from PV in the range $|z|~<~10.6$~cm. 
The VELO consists of two halves each containing 21 modules. Each module is made up of
two silicon half discs, of 300~$\mu$m thickness, with strips in either radial, $r$, or polar, $\phi$,
coordinates. The  cylindrical geometry allows 
to achieve a fast track and vertex reconstruction at the trigger level.

Since the material in front of the detector has to be minimized  in order
to reduce the multiple scattering the VELO is be placed the closest as possible to the beam pipe
(about 8~mm) during data taking. 
Silicon sensors operate inside a so called \textit{roman pot} \cite{roman}
in a secondary vacuum instead of the one in which the beams circulate, where the pressure less than $10^{-8}$~mbar.
In order to minimize the damage by irradiation and to dissipate the heat produced, a cooling
system is installed on VELO. Such a system is able to keep the temperature in a range between
-10 to 0 �C. Furthermore, the silicon discs and the frontend electronics is shielded by
an aluminium layer of 300~$\mu$m thickness (\textit{RF foil}).

\subsection{Tracking System}
The tracking system is composed by the  TT station, before the magnet, and by three stations (T1,T2,T3) after.
The TT station has a double function: together with VELO, it is used at trigger level to make transverse
momentum measurements and it is used for tracking in the event reconstruction phase.
The TT is located after the VELO and just after the RICH1 where there is a residual magnetic field
able to deflect charged particles and to make momentum measurement possible with precision about
20-30\%. TT is composed by four stations grouped in pairs, called TTa and TTb, spaced by 30 cm. The TT
are made of silicon microstrip plane modules to cover a rectangular area of 150~cm wide and 130~cm high 
corresponding to the total LHCb acceptance. The strips of the first and the fourth stations
are vertical  and measure the bending $x$ coordinate, while the
ones of the second and the third have a stereo angle of $+5$ deg and $-5$ deg respectively.

Stations T1 - T3 are placed after the magnet and consist each of an innert part (IT), closer to the beam pipe, 
and of an outer part (OT). 
 Each IT station consists
of four overlapped silicon layers with two of these that are rotate by a stereo angle of $\pm 5$ deg  and
two that are aligned to the $y$ axis. Each layer is made up by four independent
modules placed around the beam pipe, covering about a $120 \times 40$~cm$^{2}$ area (figure \ref{fig:it}).

The OT is a drift-time detector~\cite{ot}
made by straw tubes with the internal diameter of 4.9 mm filled with Ar/CO$_{2}$ gas mixture with ratio $70-30$
that provides 50 ns time resolution and 200~$\mu$m spatial resolution with 10\% maximum
occupancy. Each of the three stations is  made up by four modules (figure~\ref{fig:ot}).
In the first and third module the straw tubes are aligned to the vertical axis while in the
third and fourth ones they have a stereo angle of $\pm 5$ deg.
The total active area is about $5971 \times 4850$~mm$^{2}$ and the acceptance is
300~mrad in the horizontal plane and 250~mrad in vertical one.

The main features for the ST are listed:
\begin{itemize}
\item Spatial resolution: about 50~$\mu$m per hit both for TT and IT,
with strip pitch about 200~$\mu$m for both.
\item Hit occupancy: the average occupancy in the TT, and similarly in the IT,
varies between 1.9\% for the inner sectors to 0.2\% for the outermost modules.
\item The frontend electronics is able to form signals within 25~ns in order
to avoid overlapping between consecutive bunches.
\item As VELO is, both TT an IT are placed in a high particles rate region too.
To minimize radiation damages, sensors will work at 5�~C temperature.
\end{itemize}


\subsection{RICH system}

%%The primary role of the RICH system is to provide $\pi/K$ discrimination in a wide momentum range
%%through the Cherenkov effect. To achieve the required  separation in a momentum 
%%range between 1 and 150 GeV/c, that is the momentum range with 90\% kaons and pions
%%produced by $B$ mesons decay,  
%%Two Cherenkov detectors named RICH1 and RICH2 are used. 
RICH1 is designed to detect particles with low
and intermediate momentum value, from 1 to 40~GeV/c. 
and  is placed close to
the interaction region in order to cover the whole LHCb acceptance despite its small dimensions. It is made up by two
different radiator materials: an aerogel layer 5~cm thick whit refractive index
$n=1.03$ and a $\hbox{C}_{4}\hbox{F}_{10}$ gas layer 85~cm thick with refractive index $n=1.0014$.
The Aerogel, thanks its higher refractive index, is able to make $\pi/K$
discrimination at lower momenta, to 10~GeV/c, while the $\hbox{C}_{4}\hbox{F}_{10}$ radiator pushes
the discrimination to about 40~GeV/c.

RICH2 has a smaller angular acceptance and is placed more distant, between T3
and the first muon station M1, in order to detect forward produced particle with high momentum.
It covers an angular region of about 120~mrad in the horizontal plane and
100~mrad in the vertical one. The RICH2 is able to discriminate pions from kaon
by means $\hbox{CF}_{4}$ gas with refractive index $n=1.00046$. 

In both detectors (?)  Cherenkov photons are detected by a combined system of mirrors (both plane and spherical) used
to focus photons onto photo-detector matrices (Hybrid Photon Detector, HPD).
The light cones, because of reflection on mirrors, appears in the focal plane as circular rings
whose radius is proportional to $\theta_{c}$ angle of Cerenkov cone light. The photodetectors
are located outside the detector acceptance, in a region where the magnetic field is weak and
the radiation is not intense.

\textit{figure to be moved to performances subsection}

The Cherenkov angles for the three different materials and for different particles as a
function of the momentum are shown in figure~\ref{fig:pid_rich_2} \cite{pid3}.
\vspace{6mm}
\begin{figure}[!htbp]
\begin{center}
\includegraphics[height=5cm]{figures/pid_rich_nindex.pdf}
\end{center}
\caption{Cherenkov angles as a function of momentum for different particles
and for the three different values of the refractive index \textit{n}
corresponding to the three radiator materials used in the LHCb RICH setup.}
\label{fig:pid_rich_2}
\end{figure}

\subsection{Calorimeters}

Calorimeter system's aim is to identify hadrons, electrons and photons and to measure their energy
and position for L0 trigger, that takes a decision 4~$\mu$s after the interaction. The calorimeter
system is made up by four \textit{sub-detectors}:
\begin{itemize}
\item The scintillator Pad Detector (SPD)
\item The PreShower detector (PS)
\item The Electromagnetic Calorimeter (ECAL)
\item The Hadron Calorimeter (HCAL)
\end{itemize}
Each detector is segmented in regions in the $xy$ plane and composed by active cells with different dimensions.
ECAL, PS and SPD are divided in three sections with active pads growing from the inner to the outer
according to granularity requirements (figure~\ref{fig:cal} \textit{left}).
HCAL is divided in two sections (figure~\ref{fig:cal} \textit{right}).



The SPS and PS are placed just before ECAL. The SPD provides charged and neutral particle
separation, while PS is used for pion/electron discrimination. They are used at the
trigger level in association with ECAL to indicate the presence of electrons, photons
and neutral pions.\\
The detectors are made by two plastic scintillator layers separated
by a 15mm thick lead plate where electrons and photons radiate: the downstream sample scintillator
could so collects the radiated energy. The lead thickness is optimized to get a low
energy loss for the particles that have to be detected by ECAL. The light from scintillators
is sent to photomultipliers by wavelength-shifter (WLS) optical fibers.\\
ECAL employs the \textit{Shashlik} technology: independent modules,
made using scintillating tiles and lead plates, are alternated. Each module consists of 2~mm of lead
followed by 4~mm of scintillator material. The ECAL consists of $66$ layers of such modules
(figure~\ref{fig:ecal-hcal} right).\\
ECAL too uses WLS optical fibers to guide the light from the detector to photomultipliers
placed on the back of each module. The energy resolution achieved is
%%\begin{equation}
%%\frac{\sigma\left(E\right)}{E}=\frac{10\%}{\sqrt{E}}\oplus 1\%
%%\end{equation}
where $E$ is the energy expressed in GeV.\\
HCAL is a sampling calorimeter too: it is made up by the iron and scintillating tiles,
as absorber and active material respectively. The peculiar feature of this sampling
structure is the orientation of the scintillating: the tiles run parallel to the beam axis.


\vspace{8mm}
In the lateral direction tiles are spaced with 1~cm iron, while in the longitudinal
one the length of the tiles and iron spacers corresponds to the hadron interaction length $\lambda_{I} \simeq 20$ cm in steel.\\
The light is collected by the WLS optical fibres running along the detector towards the back
side where photomultiplier tubes are housed (figura~\ref{fig:ecal-hcal} \textit{left}).
The HCAL is used to measure the hadronic shower transverse energy for L0 requirements and
to give a contribution in improving high momentum electron/hadron separation.
The energy resolution achieved is
%%\begin{equation}
%%\frac{\sigma\left(E\right)}{E}=\frac{(69 \pm 5) \% }{\sqrt{E}}\oplus
%%(9 \pm 2)\% 
%%\end{equation}
where $E$ is the energy expressed in GeV.

\subsection{Muon System}
\label{sez:rivelatore_mu}

The Muon System  consists of five stations, 
(M1-M5, of rectangular shape. The complete system is made up by 1368 Multi Wire Proportional Chambers 
supplemented by 12 Triple GEM Chambers in the inner region of the first   station, to cope with the 
very high particle rate. The chambers employ a variety of readouts, optimized for a precise
$p_T$ measurement in the trigger. 
The complete system has an acceptance in the bending plane from 20~mrad to
306~mrad; while in the non-bending plane from 16~mrad to 258~mrad. This results in a total
acceptance of about 20\% for muons from semileptonic inclusive $b$ decays.


The  M1 station is placed in front of the calorimeters and is used in order to improve the $p_{t}$ measurement
in the trigger. M2-M5 are instead placed downstream the calorimeters and are
interleaved with 80~cm thick iron absorbers. The total absorption thickness, calorimeters included,
is about 20 interaction lengths: in this way the minimum momentum for muons
crossing the five stations is about 6~GeV/c. The geometry of the five stations is projective:
all the transverse dimensions scale as the distance from the interaction point.

Each muon station is designed to achieve an efficiency above 99\% in a 20 ns time window
with a noise rate below 1 kHz per physical channel, as
described in~\cite{muon_perf}. To reach such an efficiency four chamber layers per station are used
in M2-M5 (to layers in M1) connected in OR. The time resolution is achieved by a fast gas mixture
Ar/CO$_{2}$/CF$_{4}$ in the ratio 40:55:5. A ratio 45:15:40 is employed in the Triple GEM chambers. 






==> Chapter_2_trigger_old1.tex <==
\subsection{Trigger}
\label{sez:Trigger}

Even with the relatively large \bbbar cross-section at LHC energies 
only 1 \% of visible pp interactions result in a \bbbar event.
Moreover, only about 15\% of those events will produce at least one B-meson
with all its decay products in the acceptance of the spectrometer. The
branching fractions of decays used to study CP violation are typically less than
$10^{-3}$. In the offline selection stringent cuts have to be applied
to enhance the signal over background. Therefore 
the purpose of the LHCb trigger is to achieve the highest efficiency for the events later selected
in the offline analysis while rejecting drastically most of  uninteresting background events.
The trigger is organised in two different levels: the Level-0 (L0) trigger
based on custom electronic boards and the High-Level Trigger (HLT), implemented in a computer farm.\\
Level-0 uses the information from the calorimeter and muon systems, performing 
a selection in order to reduce the event rate from 40 MHz to below 1 MHz. The HLT is a software application running
on a processor farm [some data here] that further reduces the rate of events to be stored to about 3 kHz
(figure \ref{fig:LHCb_Trigger_RunI}).

\begin{figure}[!htbp]
\begin{center}
\includegraphics[height=8cm]{figures/LHCb_Trigger_RunI.pdf}
\end{center}
\caption{Trigger overview} \label{fig:LHCb_Trigger_RunI}
\end{figure}

\subsubsection{Level-0 hardware trigger}

The L0 trigger is divided into three independent components: the L0-Calorimeter trigger, the
L0-Muon trigger and the L0-PileUp trigger of VELO. The last is used
to reject multiple visible interactions in a  bunch crossing by means of the
\hbox{``ad hoc''} \textit{Pile-Up System} detector housed in the VELO.
The first two components are briefly described below.

\subsubsection{L0 calorimeter system}

The L0-Calorimeter part of the trigger obtains informations from the SPD, PS, ECAL and HCAL subdetectors
and computes the transverse energy deposited by incident particles: $E_{T} = E_{0} \cos \theta$ where $E_{0}$
is the energy of the particle and $\theta$ is the angle given by the cell hit in the detector.
Together with energy information, the total number of hits in the SPD (SPD Multiplicity)
is also determined in order to veto large multiplicity events that would take a too large fraction of the
available processing time in the HLT. From calorimeter informations three types of
candidates are built and selected according to specific transverse energy ($E_{T}$) criteria:
\begin{enumerate}
  \item Hadron candidate (L0Hadron)
  \item Photon candidate (L0Photon)
  \item Electron candidate (L0Electron)
\end{enumerate}\:

\subsubsection{L0 muon processors}

L0 requires a muon candidate to have a hit in all five muon stations.
The L0 muon processors boards select the two highest $p_{T}$ muon tracks in each quadrant
of the muon system with a maximum of eight candidates. The trigger sets single threshold
either on the largest muon $p_{T}$ (L0 muon trigger) or on the product of the largest and the 2nd largest
(L0 dimuon trigger).


Events with SPD multiplicity > 600 are excluded in the L0 muon trigger in order to minimize the track multiplicity.
This limit is raised to 900 in the L0 dimuon trigger for a small increase in rate.
[wonder if this is already covered in the calo trigger]
\\\:
The typical L0 thresholds used in Run I are listed in the table \ref{tab:L0thresh} \cite{TriggRunI}.
[to see if the table is really necessary].

The total output rate of the L0 trigger is limited to 1 MHz, which is the maximum rate
value accepted by the HLT1. Such output rate consists of about
400 kHz of muon triggers, about 500 kHz of hadron triggers and about 150 kHz of electron and photon
triggers (the individual triggers have an overlap of about $10\%$).

\subsection{High Level Trigger}

Data from L0 are send to the Event Filter computer Farm (EFF) which runs the HLT algorithms.
The HLT is a software application whose $29500$ instances run
on the EFF. Each instance is made up of independently operating trigger lines: each line
consists of selection parameters for a specific class of events.\\
The HLT is divided into two stages. The first stage (HLT1) processes the full L0 rate and uses
partial event reconstruction to reduce the rate to about 40 kHz. The second stage (HLT2) reduces the rate to
about 3 kHz performimg a more complete event reconstruction \cite{mu_trig}.

\subsubsection{HLT1}

The offline VELO reconstruction algorithm performs a full 3D pattern recognition
and is fast enough to be run on all events entering the HLT. However, it
makes a second pass on unused hits to enhance the efficiency for tracks pointing far away
from the beam-line. In the first stage of the HLT this second pass is not used because of CPU constraints.
Vertices are reconstructed from a minimum of five intersecting VELO tracks and are considered
to be ``primary vertices'' when are in a radius of 300 $\mu m$ of the mean position of the $pp$-interaction envelope.
HLT1 limits the number of VELO tracks that are passed through the forward tracking
algorithm (that searches for matching hits in the tracking stations).
The forward track search has further a minimum momentum requirement, between 3 and
6 GeV/c during Run I [what about Run II?]. If a VELO track without matching muon hits occurs, then a minimum $p_{T}$
between 0.5 and 1.25 GeV/c is required. The reconstructed forward tracks are then fitted.\\
For comparison, with this procedure a resolution of only 3\% worse than the 15.1 MeV/$c^{2}$
obtained offline is found for the invariant mass of
$J/\psi \rightarrow \mu^{+} \mu^{-}$ candidates reconstructed. For muon candidates the offline muon
identification algorithm \cite{mu_perf} is applied, so the purity of the muon sample is increased.\\

The inclusive beauty and charm trigger selection is based on track $p_{t}$
and on displacement from the primary vertex (typical value IP > 0.1 mm). This trigger line
produces around 58 kHz of output: the largest contribution to the allocated HLT1
bandwidth. It is the most efficient line for physics channels that do not contain leptons in
the final state. The inclusive one-track based trigger also exists in a version for electrons or photons
identified by L0, with reduced thresholds related to the inclusive version. The output rate of these
lines is around 7 kHz.\\

A similar line exists for tracks that are matched to hits in the muon chambers.
Such trigger line is able to select those good quality muon candidates that are detached
from the primary vertex and that have $p_{T} > 1 \hbox{GeV}/c$; whereas single muon candidates with
$p_{T} > 4.8 \hbox{GeV}/c$ are selected by a trigger line without any vertex separation
requirements.\\

Dimuon candidates are either selected based on their mass values: if $m_{\mu \mu} > 2.5 \hbox{GeV}/c^{2}$ the
selection in made without any displacement requirement, otherwise it is based on their displacement without the mass requirement.
Dimuon candidates are also triggered based on their distance of closest approach (DOCA): the distance of closest approach of two objects
is defined as the distance between their centers when they are externally tangent and can be referred to
objects with geometric shapes or physical particles with well defined boundaries.\\
After the combination of the muon trigger lines, a 14 kHz output rate is obtained.\\
Dedicated lines are developed in order to improve the trigger performance in case of the presence
of events containing candidates for displaced vertices, high ET jets, di-protons or high $p_{T}$ electrons.
Luminosity and beam-gas measurements could be selected by additional lines used in the HLT1.\\

HLT1 muon lines are executed only if events have passed L0Muon or L0DiMuon. They are divided in sigle
and dimuon lines: Hlt1TrackMuon accepts events with B, D or $\tau$ decays with at least one muon in the final state,
Hlt1SingleMuonHighPT triggers on muons originating from heavy particles with a negligible lifetime like
$W^{\pm}$ or $Z^{0}$, Hlt1DiMuonHighMass selects $b$-hadron decays without lifetime cuts,
Hlt1DiMuonLowMass triggers on final states with two muons with a relatively small invariant mass.\\


\subsubsection{HLT2}

The HLT2 is able to reduce the rate down to $\sim3$ kHz: at this rate HLT2 performs
forward tracking of all VELO tracks. HLT2 employs the algorithm based on seeding the search with VELO tracks.
In order limit the search windows $p > 5 \hbox{GeV}/c$ and $p_{T} > 0.5 \hbox{GeV}/c$ cuts are applied.\\
Muon identification is performed using the off-line algorithm on all tracks from the forward
tracking. Tracks are also associated to ECAL clusters to identify electrons.\\
Informations from the L0-Calorimeter system are used to build photons and neutral pions.\\
The HLT2 is made up by:
\begin{itemize}
\item \textbf{Generic beauty trigger}: a large portion of the 3 kHz output rate of HLT2
is selected by \textit{topological} trigger lines, which
are designed to trigger on partially reconstructed inclusive $b$-hadron decays. Such kind
of lines are used to cover all $b$-hadrons with at least two charged particles in the final state and
a displaced decay vertex. The track selection is based on requirements on track fit quality
($\chi^{2} / ndof$), impact parameter (IP) and identification of muons or electrons.
\hbox{N-body} vertexes are constructed, starting from the selected tracks, by requiring their distance of
closest approach (DOCA), while $n$-track combination uses the variables: $\sum |p_{T}|$, $p_{T}^{min}$,
$n$-body invariant mass ($m$), DOCA, $\hbox{IP}\chi^{2}$ and flight distance (FD) $\chi^{2}$.
The output rate of the topological trigger is 2 kHz.

\item \textbf{Muon triggers}: are designed to select events containing muon or dimuon candidates.
The single muon candidate event is selected by two different lines:
the first one, called Hlt2SingleMuon, selects semileptonic $b$ and $c$-hadron decays
with the TOS condition\footnote{An event is classified as TOS (Trigger on Signal) if
the trigger objects that are associated with the signal are sufficient to trigger the event.
An event is classified as TIS (Trigger Independent of Signal) if it could have been triggered
by those trigger objects that are not associated to the signal.};
the second one, Hlt2SingleMuonHighPT, is designed to select heavy particles, like $W^{\pm}$ and
$Z^{0}$, that decay promptly to one or more muons.\\
The Dimuon candidates selection is grouped in two categories:
the ones dedicated to prompt decays use the mass as the main discriminant, while detached
lines use the separation between the dimuon vertex and the PV as the main discriminant.
The first group is formed by Hlt2DiMuonJPsi(Psi2S) and Hlt2DiMuonJPsi(Psi2S)HighPT lines.\\
The second one is made by Hlt2DiMuonDetached, Hlt2DiMuonDetachedHeavy and Hlt2DiMuonDetachedJPsi
lines.\\
Such lines are optimized in order to take advantage of the physics potential of $J/\psi$ and
$B \rightarrow J/\psi X$ decays.\\
The total output rate of all single and dimuon trigger lines is about 1 kHz.
\item \textbf{Charm triggers}: about 600 kHz of $c\overline{c}$-events are produced in the 2012
in the LHCb acceptance, so tight exclusive selections are required.
Hadronic two and three body lines are the main exclusive selections for prompt charm.
The total output rate of all charm selections is about 2 kHz.
\end{itemize}\:



\clearpage


==> Chapter_2_trigger_old2 <==
\subsection{Trigger}
\label{sez:Trigger}

Even with the relatively large $\bbbar$ cross-section at LHC energies 
only 1 \% of visible pp interactions result in a $\bbbar$ event.
Moreover, only about 15\% of those events will produce at least one B-meson
with all its decay products in the acceptance of the spectrometer. The
branching fractions of decays used to study CP violation are typically less than
$10^{-3}$. In the offline selection stringent cuts have to be applied
to enhance the signal over background. Therefore 
the purpose of the LHCb trigger is to achieve the highest efficiency for the events later selected
in the offline analysis while rejecting drastically most of  uninteresting background events.
The trigger is organised in two different levels: the Level-0 (L0) trigger
based on custom electronic boards and the High-Level Trigger (HLT), implemented in a computer farm.\\
Level-0 uses the information from the calorimeter and muon systems, performing 
a selection in order to reduce the event rate from 40 MHz to below 1 MHz. The HLT is a software application running
on a processor farm [some data here] that further reduces the rate of events to be stored to about 3 kHz
(figure \ref{fig:LHCb_Trigger_RunI}).

\begin{figure}[!htbp]
\begin{center}
\includegraphics[height=8cm]{figures/LHCb_Trigger_RunI.pdf}
\end{center}
\caption{Trigger overview} \label{fig:LHCb_Trigger_RunI}
\end{figure}

\subsubsection{Level-0 hardware trigger}

The L0 trigger is divided into three independent components: the L0-Calorimeter trigger, the
L0-Muon trigger and the L0-PileUp trigger of VELO. The last is used
to reject multiple visible interactions in a  bunch crossing by means of the
\hbox{``ad hoc''} \textit{Pile-Up System} detector housed in the VELO.
The first two components are briefly described below.

\subsubsection{L0 calorimeter system}

The L0-Calorimeter part of the trigger obtains informations from the SPD, PS, ECAL and HCAL subdetectors
and computes the transverse energy deposited by incident particles: $E_{T} = E_{0} \cos \theta$ where $E_{0}$
is the energy of the particle and $\theta$ is the angle given by the cell hit in the detector.
Together with energy information, the total number of hits in the SPD (SPD Multiplicity)
is also determined in order to veto large multiplicity events that would take a too large fraction of the
available processing time in the HLT. From calorimeter informations three types of
candidates are built and selected according to specific transverse energy ($E_{T}$) criteria:
\begin{enumerate}
  \item Hadron candidate (L0Hadron)
  \item Photon candidate (L0Photon)
  \item Electron candidate (L0Electron)
\end{enumerate}\:

\subsubsection{L0 muon processors}

L0 requires a muon candidate to have a hit in all five muon stations.
The L0 muon processors boards select the two highest $p_{T}$ muon tracks in each quadrant
of the muon system with a maximum of eight candidates. The trigger sets single threshold
either on the largest muon $p_{T}$ (L0 muon trigger) or on the product of the largest and the 2nd largest
(L0 dimuon trigger).


Events with SPD multiplicity > 600 are excluded in the L0 muon trigger in order to minimize the track multiplicity.
This limit is raised to 900 in the L0 dimuon trigger for a small increase in rate.
[wonder if this is already covered in the calo trigger]
\\\:
The typical L0 thresholds used in Run I are listed in the table \ref{tab:L0thresh} \cite{TriggRunI}.
[to see if the table is really necessary].

The total output rate of the L0 trigger is limited to 1 MHz, which is the maximum rate
value accepted by the HLT1. Such output rate consists of about
400 kHz of muon triggers, about 500 kHz of hadron triggers and about 150 kHz of electron and photon
triggers (the individual triggers have an overlap of about $10\%$).

\subsection{High Level Trigger}

Data from L0 are send to the Event Filter computer Farm (EFF) which runs the HLT algorithms.
The HLT is a software application whose $29500$ instances run
on the EFF. Each instance is made up of independently operating trigger lines: each line
consists of selection parameters for a specific class of events.\\
The HLT is divided into two stages. The first stage (HLT1) processes the full L0 rate and uses
partial event reconstruction to reduce the rate to about 40 kHz. The second stage (HLT2) reduces the rate to
about 3 kHz performimg a more complete event reconstruction \cite{mu_trig}.

\subsubsection{HLT1}

The offline VELO reconstruction algorithm performs a full 3D pattern recognition
and is fast enough to be run on all events entering the HLT. However, it
makes a second pass on unused hits to enhance the efficiency for tracks pointing far away
from the beam-line. In the first stage of the HLT this second pass is not used because of CPU constraints.
Vertices are reconstructed from a minimum of five intersecting VELO tracks and are considered
to be ``primary vertices'' when are in a radius of 300 $\mu m$ of the mean position of the $pp$-interaction envelope.
HLT1 limits the number of VELO tracks that are passed through the forward tracking
algorithm (that searches for matching hits in the tracking stations).
The forward track search has further a minimum momentum requirement, between 3 and
6 GeV/c during Run I [what about Run II?]. If a VELO track without matching muon hits occurs, then a minimum $p_{T}$
between 0.5 and 1.25 GeV/c is required. The reconstructed forward tracks are then fitted.\\
For comparison, with this procedure a resolution of only 3\% worse than the 15.1 MeV/$c^{2}$
obtained offline is found for the invariant mass of
$J/\psi \rightarrow \mu^{+} \mu^{-}$ candidates reconstructed. For muon candidates the offline muon
identification algorithm \cite{mu_perf} is applied, so the purity of the muon sample is increased.\\

The inclusive beauty and charm trigger selection is based on track $p_{t}$
and on displacement from the primary vertex (typical value IP > 0.1 mm). This trigger line
produces around 58 kHz of output: the largest contribution to the allocated HLT1
bandwidth. It is the most efficient line for physics channels that do not contain leptons in
the final state. The inclusive one-track based trigger also exists in a version for electrons or photons
identified by L0, with reduced thresholds related to the inclusive version. The output rate of these
lines is around 7 kHz.\\

A similar line exists for tracks that are matched to hits in the muon chambers.
Such trigger line is able to select those good quality muon candidates that are detached
from the primary vertex and that have $p_{T} > 1 \hbox{GeV}/c$; whereas single muon candidates with
$p_{T} > 4.8 \hbox{GeV}/c$ are selected by a trigger line without any vertex separation
requirements.\\

Dimuon candidates are either selected based on their mass values: if $m_{\mu \mu} > 2.5 \hbox{GeV}/c^{2}$ the
selection in made without any displacement requirement, otherwise it is based on their displacement without the mass requirement.
Dimuon candidates are also triggered based on their distance of closest approach (DOCA): the distance of closest approach of two objects
is defined as the distance between their centers when they are externally tangent and can be referred to
objects with geometric shapes or physical particles with well defined boundaries.\\
After the combination of the muon trigger lines, a 14 kHz output rate is obtained.\\
Dedicated lines are developed in order to improve the trigger performance in case of the presence
of events containing candidates for displaced vertices, high ET jets, di-protons or high $p_{T}$ electrons.
Luminosity and beam-gas measurements could be selected by additional lines used in the HLT1.\\

HLT1 muon lines are executed only if events have passed L0Muon or L0DiMuon. They are divided in sigle
and dimuon lines: Hlt1TrackMuon accepts events with B, D or $\tau$ decays with at least one muon in the final state,
Hlt1SingleMuonHighPT triggers on muons originating from heavy particles with a negligible lifetime like
$W^{\pm}$ or $Z^{0}$, Hlt1DiMuonHighMass selects $b$-hadron decays without lifetime cuts,
Hlt1DiMuonLowMass triggers on final states with two muons with a relatively small invariant mass.\\


\subsubsection{HLT2}

\textbf{THIS SUBSECTION HAS TO BE REVISED AND SHORTENED}
\\
The HLT2 is able to reduce the rate down to $\sim3$ kHz: at this rate HLT2 performs
forward tracking of all VELO tracks. HLT2 employs the algorithm based on seeding the search with VELO tracks.
In order limit the search windows $p > 5 \hbox{GeV}/c$ and $p_{T} > 0.5 \hbox{GeV}/c$ cuts are applied.\\
Muon identification is performed using the off-line algorithm on all tracks from the forward
tracking. Tracks are also associated to ECAL clusters to identify electrons.\\
Informations from the L0-Calorimeter system are used to build photons and neutral pions.\\
The HLT2 is made up by:
\begin{itemize}
\item \textbf{Generic beauty trigger}: a large portion of the 3 kHz output rate of HLT2
is selected by \textit{topological} trigger lines \bf{(check if the LINES term has been defined)}, which
are designed to trigger on partially reconstructed inclusive $b$-hadron decays. Such kind
of lines are used to cover all $b$-hadrons with at least two charged particles in the final state and
a displaced decay vertex. The track selection is based on requirements on track fit quality
($\chi^{2} / ndof$), impact parameter (IP) and identification of muons or electrons.

%%
%%\hbox{N-body} vertexes are constructed, starting from the selected tracks, by requiring their distance of
%%closest approach (DOCA), while $n$-track combination uses the variables: $\sum |p_{T}|$, $p_{T}^{min}$,
%% $n$-body invariant mass ($m$), DOCA, $\hbox{IP}\chi^{2}$ and flight distance (FD) $\chi^{2}$.
%%The output rate of the topological trigger is 2 kHz.

\item \textbf{Muon triggers}: are designed to select events containing muon or dimuon candidates.
  The single muon candidate event is selected by two different lines:
the first one, called Hlt2SingleMuon, selects semileptonic $b$ and $c$-hadron decays
with the TOS condition\footnote{An event is classified as TOS (Trigger on Signal) if
the trigger objects that are associated with the signal are sufficient to trigger the event.
An event is classified as TIS (Trigger Independent of Signal) if it could have been triggered
by those trigger objects that are not associated to the signal.};
the second one, Hlt2SingleMuonHighPT, is designed to select heavy particles, like $W^{\pm}$ and
$Z^{0}$, that decay promptly to one or more muons.\\
The Dimuon candidates selection is grouped in two categories:
the ones dedicated to prompt decays use the mass as the main discriminant, while detached
lines use the separation between the dimuon vertex and the PV as the main discriminant.
The first group is formed by Hlt2DiMuonJPsi(Psi2S) and Hlt2DiMuonJPsi(Psi2S)HighPT lines.\\
The second one is made by Hlt2DiMuonDetached, Hlt2DiMuonDetachedHeavy and Hlt2DiMuonDetachedJPsi
lines.\\
Such lines are optimized in order to take advantage of the physics potential of $J/\psi$ and
$B \rightarrow J/\psi X$ decays.\\
The total output rate of all single and dimuon trigger lines is about 1 kHz.
\item \textbf{Charm triggers}: about 600 kHz of $c\overline{c}$-events are produced in the 2012
in the LHCb acceptance, so tight exclusive selections are required.
Hadronic two and three body lines are the main exclusive selections for prompt charm.
The total output rate of all charm selections is about 2 kHz.
\end{itemize}\:



\clearpage


==> Introduction_old.tex <==


\section{Introduction}

\lhcb is an experiment at the CERN \lhc, dedicated to the study of heavy flavours with large statistics. 
The resulting high precision makes possible the observation of tiny deviations from the predictions of the Standard Model  (SM)
in \CP violation and rare
phenomena, variations which could hint at New Physics (NP) processes.
% \lhcb is installed at the CERN  LHC machine. 
\lhcb started taking data in 2010. The so-called Run~1 
commenced at an initial centre of mass energy of  $\sqrt{s}=7$ TeV which was then increased to $\sqrt{s}=8$ TeV,
collecting an integrated luminosity of $3.23\,\invfb$ until the end of 2012.
After a two-year shutdown, \lhc operation continued from 2015 to 2018 (Run~2), when the experiment
took data at $\sqrt{s}=13$ TeV, recording an integrated luminosity of $\sim 6 \,\invfb$. Throughout the running periods,
\lhcb collected and analysed an unprecedented number of $\bquark$ decays, and also enlarged its
scope to include charm physics, $W$ and $Z$ measurements, jets and nuclear collisions. 

In this paper the motivation for the \lhcb
experiment is described,  recalling how its design was
developed and evolved. The experiment's major achievements in terms of physics results are then summarised. 
Finally we discuss the plans for the future upgrade, in the period when the Super-KEKB collider will also operate. 
%\cite{BELLE_operation}. 

The layout of this paper is as follows.
The Introduction (Sect. 1) describes the status of the $\bquark$ physics programme at the time the \lhcb detector was conceived, and provides an evolution of its design. 
In Sect. 2 
%ref\{????? add here hthe label of the concerned section.
the basic elements of the detector are described,  optimised for the requirements of heavy-flavour physics measurements, together 
with a description of the triggers.
%ref\{????? add here hthe label of the concerned section.
The measurements which were originally the major aims of the experiment,
i.e. the CKM matrix measurements and \CP violation 
 and  very rare decays  
%ref\{????? add here hthe label of the concerned section.
of the $b$-quark, are reviewed in Sects. 3 and 4, respectively.
In Sect. 5,
%ref\{????? add here hthe label of the concerned section.
a summary of the wide-ranging results in $\bquark$- and $\cquark$- spectroscopy is presented.
%ref\{????? add here hthe label of the concerned section.
A review is given of the many {\it {non planned}} physics areas in Sect. 6, such as results on jets,  electro-weak (EW) physics, and searches for new particles not associated with heavy flavours.
In all these domains, \lhcb proves to be an extremely versatile detector, providing complementary measurements to those of the \lhc General Purpose Detectors (GPDs).
% produced in the years 2010-2018 at LHC.
The paper concludes in Sect. 8 with a short description of the 
upgrade plans, which will ensure \lhcb operation beyond 2030.

The choice of physics results presented in this paper cannot possibly cover all domains in which \lhcb has produced valuable measurements, in particular improving existing results or providing the best single measurements with respect to world averages.
\textcolor{red} {
The paper presents the authors' subjective summary of \lhcb's
many major achievements, however the review 
inevitably omits a substantial number of important measurements. 
To this end, additional information 
can  be found in the paper's exhaustive bibliography.}
%The wide bibliography of \lhcb publications  supplied herein can provide the reader with more detail in the appropriate areas of interest.  
  
\subsection{$\bquark$ physics at the end of the XXth century}

In 1970 Glashow, Iliopoulos and Maiani postulated the existence of a fourth
quark, {\em charm},  necessary to explain the smallness
of $\Kz$ oscillations in the framework of the 
Standard Model of Weak Interactions~\cite{Glashow:1970gm}. 
The so-called Glashow-Iliopoulos-Maiani (GIM) mechanism mechanism generalized
Cabibbo's idea of rotated  weak currents to the quark model with two doublets, 
introducing a $2 \times 2$ mixing matrix written in terms of the Cabibbo angle. 
An experimental confirmation of the fourth quark hypothesis came in 1974 with the discovery of $\jpsi$~\cite{Augustin:1974xw, Aubert:1974js}, soon
identified as a $\ccbar$ bound state, and followed by the discovery of open charm. 
In 1973 Kobayashi and Maskawa \cite{Kobayashi:1973fv}
proposed a third heavy-quark doublet 
in order to describe  \CP violation in the framework of the SM, thus 
generalizing the Cabibbo matrix to the $3 \times 3$ CKM (Cabibbo, Kobayashi, Maskawa) matrix. 
The  discovery of the $\PUpsilon$ in 1975, followed by the charged and neutral $\B$-mesons in 1983 
\cite{Behrends:1983er} 
 proved the validity of their idea and held the  
prospect of understanding quantitatively \CP violation.

The level of \CP violation  in
$\bquark$ quark decays  was expected to be orders of magnitude larger than in the neutral $\kaon$ system, but
unfortunately the relevant decay channels had only tiny branching fractions, so the  lack of intense
``$\bquark$-quark sources''  slowed the progress  of beauty physics: in particular, in 1986 the PDG  only listed five decay modes of $\Bz$ and $\Bpm$.
%% It was soon established that the most promising decay channel
%% to look for CP violation and quantitatively test
%% the theoretical predictions was $B^0 \rightarrow J/\psi K_S$. 
However in 1987 a new impetus came from the discovery at ARGUS of
$\B^0 - {\overline{\B}^0}$  oscillations
 \cite{Schroder:1987vf}.
It was clear that the forthcoming LEP machine,
designed for an entirely different purpose, 
and the symmetrical CESR collider, could not 
yield an exhaustive answer to all the questions related to the CKM hypothesis,
despite their valuable contributions to many facets of $\bquark$-physics
\cite{Abbaneo:2000ej,doi:10.1146/annurev-nucl-010609-115108}. 
When in 1989 P. Oddone proposed an asymmetric $\epem$ collider \cite{Oddone:1989ir} operating at the $\PUpsilon(4S)$ energy with a
luminosity above  $ \plum{33}$, an intense period of accelerator studies ensued. This gave birth to the PEP-II and KEKB $\PB$ Factories, which were approved in 1994, 
and  started operating in 1998, soon reaching and passing  their 
design luminosity. 

Around this time, proponents pursued the idea of exploiting hadron beams to attack
the problem of detecting \CP violation in the $\bquark$ sector. 
The idea behind this was that the large hadronic $\bquark$ production cross-section plus the high-intensity hadron beams at the already existing and planned proton accelerators
would  produce a large number of $\bbbar$ pairs, sufficient to gather evidence for \CP violation
at least in the so-called ``golden channel'' $\Bz \to \jpsi \KS$.
To achieve an adequate background
rejection, the experimental difficulties were formidable because of the small ratio of the $\bquark$ cross-section 
to the total hadronic cross-section at the $\sqrt{s}$ values available in fixed-target and collider experiments. 
 In 1985, the fixed-target WA75 experiment  at the CERN SPS \cite{Albanese:1985wk}
 observed the first   partially reconstructed $\bbbar$ pair produced by an extracted pion beam 
 of 350 GeV/c, confirming that the production cross-section at such low energies was very small. 
 To circumvent this problem, impractical experiments were proposed 
 \cite{Fidecaro:1990py} 
 for the CERN SPS and for the planned UNK machine at Serpukhov, 
 with a brute-force approach based on a high-intensity extracted beam and a minimalist detector designed 
 to reconstruct the  $\Bz \to \jpsi \KS$ decay and to provide flavour tagging. This was without 
 time-dependent analysis of the decay since the beam-dump character of the experiments made the use
 of a micro vertex detector impossible. There were exploratory
 fixed-target experiments, at CERN (WA92) \cite{Adamovich:1996ih} 
 and at Fermilab (E653, E672, E771, E789)  \cite{Mishra:1993hn}, which tried to observe and measure beauty events,  albeit without (or very limited) success.

 At the time when the $\epem$ colliders were approved,
the HERA-B experiment had been conceived at DESY \cite{Krizan:1994ts}. 
Approved in 1994, HERA-B exploited the 920 GeV HERA proton beam
on a fixed target made of metallic wires, placed  inside Roman Pots in the vacuum pipe, and immersed in the beam halo. 
HERA-B was approved to take data in 1998, one year before PEP-II and KEKB. 
The sophisticated apparatus, a single-arm spectrometer, included a RICH,
a large microvertex silicon detector, a high-resolution tracker, 
plus an electromagnetic calorimeter.
HERA-B was designed primarily for the detection of the  
$\Bz \to \jpsi \KS$ decay and its trigger was based on  $\jpsi$ reconstruction at the first level. 

At $\sqrt{s}=40$ GeV, the $\bbbar$
cross-section is about $10^{-6}$ of the total hadronic cross-section, hence HERA-B had to achieve
a background rejection around $10^{-11}$ for the 
$\Bz \to \jpsi \KS$ decay. 
 Data taking conditions were similar to those of the current \lhcb experiment (a 40 MHz interaction rate), as were the requirements of radiation resistance. 
 HERA-B started data taking in 2000 but it soon emerged that 
 the detector did not have sufficient rejection power against background and the track reconstruction 
 %both offline and online 
 was not as efficient as expected.
 %Also, 
 The large number of 
 detector stations and their total thickness  in terms of radiation lengths made secondary interactions 
 an important 
 %major
 issue for event reconstruction. Eventually  HERA-B could not observe $\bquark$ events efficiently, but taught several valuable lessons to be learn for any experiment in a crowded hadron-collision 
 environment: the need of a robust and efficient tracking and flexible trigger systems to adapt to 
 harsher environments than may have been expected, as well as the 
 need to design the thinnest and lightest detector (in terms of radiation and interaction lenghts).
% , in 
%a crowded hadron-collision environment, the thinnest and lightest  detector (in terms of radiation and %interaction lengths) is mandatory.

\subsection{Towards the \lhc}
Over the same period, the planned \lhc and SSC machines, with their
large energies,  promised spectacular increases
of the $\bbbar$ cross-section, thus making the task of
background rejection much simpler. 
This was particularly true for operation in collider mode,
but even in fixed-target mode the $\bquark$ cross-section was
expected to be a respectable $1 ~\mu$b at the \lhc and $2 ~\mu$b at
the SSC \cite{Berger:1993yw}. 
The large cross-section and corresponding good
background rejection would facilitate a hadron \bfactory competitive and complementary with
$\epem$  colliders, which could focus primarily on the measurement 
of \CP violation but would also allow  the study of the spectrum
of all $\bquark$ particles.  Given the intrinsically 
``democratic'' nature of hadronic production, the new hadron machines would also give access
to large samples of $\Bs$ and of $b$ baryons, something
not possible at $\epem$ colliders operating at the $\PUpsilon$ resonances. 
  
Two schools of thought soon emerged: one pursuing a fixed-target  strategy
and the other based on collider mode. The more favourable ratio of
the $\bbbar$ to the total hadronic cross-section, about two orders
of magnitude larger in collider mode,  gave this a competitive advantage.
This was however  partially offset by the larger event multiplicity
and by the shorter flight path of beauty particles. 
Active silicon targets were also possible with an extracted beam. 
Kinematically, $\bbbar$ production is forward peaked in the centre-of-mass (CM) system,
but the CM Lorentz boost in fixed target mode concentrates the event at smaller angles
than in collider mode. It was therefore possible, in principle,  to build a more
compact detector,  achieving larger angular acceptance at lower cost.
That was an important aspect, since a
dedicated $\B$ experiment at \lhc (or SSC) was considered somewhat peripheral  with respect to the general-purpose experiments.
%, and  the cost issue played an important role
There was also the
possibility of recycling components (in particular dipole magnets) from existing detectors. 

Another reason in favour of the fixed-target concept
was that a  collider
$\PB$ experiment could not operate at the design luminosity of the machine
($10^{33-34})$ because of the significant number of 
overlapping interactions (pile-up).
Prior to the realisation that the individual experiment luminosity could be tuned
over a broad range,  this would have
required dedicated low-luminosity 
running, creating a potential conflict with the major experiments and considerably
reducing the data-taking time. 

The anticipated  demise of the SSC  led three groups to study and propose dedicated
$\bquark$ experiments at the \lhc. The three Letters of Intent (LoI)  were presented in 1993. 
COBEX \cite{Erhan:1994tt}, an acronym for Collider Beauty Experiment,
with P. Schlein as spokesperson, was a collider experiment with
a backward-forward geometry. The other two proposals,
Gajet \cite{Dauncey:1994vn} (spokesperson T. Nakada) and LHB \cite{Waldi:1994jx} (spokesperson G. Carboni)
were fixed target experiments, the first,
as the name suggests, using a gas jet target, the latter exploiting an extracted beam. 
Since no traditional beam extraction was foreseen for the \lhc, LHB (Large Hadron Beautyfactory) 
used a parasitic extraction technique, based on crystal channeling.
A dedicated R\&D experiment, RD22, was approved to test the feasibility of this idea at the SPS, demonstrating
that high-efficiency beam extraction (larger than 10\%) was possible \cite{Akbari:1993mb}.
The three proposed experiments 
were presented in their final form in 1994 at the Beauty'94 Conference~\cite{Schlein:1994kqa}. 
It should also be noted that, by then, CDF had already 
contributed important $\bquark$-physics results, offering a glimpse of what would later prove to be the extraordinary
success of $b$-physics at hadronic machines. 

Following the submission of the LoIs, the \lhc Committee (LHCC) issued its recommendation: 
``the collider model approach has the greater potential in view of the very high rate of $\bquark$ production, the much better
signal/background ratio and the possibility of exploring other physics in the forward direction at 14 TeV''. The 
LHCC  encouraged the three collaborations to join together and design a new experiment, incorporating attributes of each, and operating in collider mode. The LHCC noted that 
its ambitious request was justified by the fact that, at the startup of the \lhc, the  experiment
would not be an exploratory one, since \CP violation would already have been observed 
``at HERA-B, FNAL or \bfactories'' (in fact this happened
only for the \bfactories).  
The LHCC also issued guidelines requiring a number of issues to be
addressed and solved. The three experiments gave birth to the new
LHC-B Collaboration (then named), which published its Letter of Intent in 1995~\cite{Dijkstra:1995cha}.

Soon afterwards, a competing $\B$-physics  
experiment, BTeV~\cite{Kulyavtsev:2000zz}, was proposed to run at the Fermilab Tevatron, incorporating  a single magnet, a double arm spectrometer and a vertex trigger at the first level, in order to recover the reduced $\bquark$  production cross section. Following the decision to shut down the Tevatron, BTeV was not approved, however several of the experiment's innovative ideas were carried through to the future \lhcb experiment.









==> Lhcbdet_old.tex <==



\section{ The LHCb Detector}
The basic mechanism for heavy-quark production at LHC is via gluon-gluon fusion. The $\ccbar$ 
or $\bbbar$ pairs angular distribution is peaked at small angles with respect to the 
beam line, with high correlation between the constituents of the pair. This allows to detect with good 
acceptance the
resulting hadrons in a rather limited solid angle. QCD calculations give cross-section values 
$\sigma_{\ccbar} \simeq 1.5$ mb and $\sigma_{\bbbar} \simeq 0.5$ mb respectively. 
The event multiplicity is large requiring a high granularity of the detector, together with a 
minimal thickness in terms of radiation and interaction lengths to minimize secondary interactions. 
The Letter of Intent of LHC-B presented a forward spectrometer with 400 mrad acceptance and a single 
large dipole magnet. The 
apparatus would fit inside the former DELPHI cavern at LEP with little modifications to the 
existing infrastructure but, for reasons of cost, 
the detector sacrificed half of the solid angle. The LOI design 
 borrowed several solutions from the three ancestor experiments and from the contemporary
HERA-B, which had rate and radiation issues close to those expected at LHC.  In addition to the
latter experiment,  LHC-B had in addition a hadron calorimeter and a second RICH with two radiators. 
Initially it was thought that an efficient tracking system in a harsh environment would require a large number 
of tracking stations, so, paralleling HERA-B,  LHC-B had 12 tracking stations in the large-angle region. This
number was reduced to 10 in the Technical Proposal presented in 1998 by the Collaboration,
which by then changed its name to LHCb. The bad performance of HERA-B. also ascribed to the 
large amount of material in the detector, prompted LHCb to perform a thorough review of the 
apparatus, with the eye to reducing material without sacrificing performances. A Technical Design Report 
issued in 2003 presented the Reoptimized Detector,which was eventually built and is briefly presented in the following
subsections. 

%\input{Chapter_2_detector.tex}

%%\input{Chapter_2_trigger.tex}

\newpage















==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

# Make the upright version
upright: 
	$(BUILDCOMMANDUPRIGHT)



==> abstract_EPJH.tex <==
In this paper we will describe the fantastic success of the experiment LHCb, which was initially planned to be dedicated to the $b$-physics, in particular to CP violation studies and $b$ very rare decays.

\noindent After the first data collected, 
in 2012, 
it became clear the tremendous potentiality of the LHCb detector for the $c$-physics, also in term of CP violation and rare decays.

\noindent Later it was found that also Electroweak physics, jets studies and even new particles searched in open states, were not only possible, but favoured by the excellent capability of the detector to identify muons and to reconstruct separate verteces close to the primary $pp$ interaction.

\noindent At the end of Run 2, i.e. data taken until 2018 (when LHC stopped for a long shut down), LHCb essentially had set the CKM quark mixing matrix elements concernig
$b$ and $c$ quarks, measured Standard Model decays of $b$ and $c$ quarks 
expected of the order of 10$^{-9}$-$10^{-11}$,
improved the $b$ and $c$ spectroscopy knowldge adding several new quark states, and many other high value measurements.

It is impossible to describe all these important measurements: in this paper we make a selection just to give the idea of the extremely wide domain of succesfull physics measurements that LHCb accomplished. The selection is clearly subjective and reflects the authors' choices.



==> dark-sector_old.tex <==


\paragraph{Dark Photons.}
%\subsubsection{Dark Photons.}
%=====================================================================
%dall'articolo: LHCb collaboration, R. Aaij et al., Search for dark photons produced in 13 TeV pp collisions, Phys. Rev. Lett. 120 (2018) 061801, arXiv:1710.02867.
The possibility that dark matter particles may interact via unknown forces, 
felt only feebly by Standard Model (SM) particles, has motivated substantial 
effort to search for dark-sector forces (see \cite{DM-review} for a review). 
A dark-force scenario involves a massive dark photon, $A^{\prime}$, 
whose coupling to the electromagnetic current is suppressed relative to that of the
 ordinary photon, $\gamma$, by a factor of $\epsilon$. 
In the minimal model, the dark photon 
does not couple directly to charged SM particles; however, a coupling may arise
 via kinetic mixing between the SM hypercharge and $A^{\prime}$~field strength tensors. 
%\cite{} [2–7]. 
This mixing provides a potential portal through which dark photons may be produced if kinematically allowed. 
If the kinetic mixing arises due to processes whose amplitudes involve one or two loops containing high-mass particles, perhaps even at the Planck scale, 
then   $10^{-12} \leq   \epsilon^2 \leq 10^{-4}$ is expected 
\cite{DM-review}. 
 Fully exploring this few-loop range of kinetic-mixing strength is an important goal of dark-sector physics.
Constraints have been placed on visible $A^{\prime}$~decays by previous beam-dump 
%\cite{}[7–21],
 fixed-target 
%\cite{}[22–24], 
collider 
%\cite{}[25–28], 
and rare-meson-decay 
%\cite{}[29–38] 
experiments. 
The few-loop region is ruled out for dark photon masses $m(A^{\prime})\sim10\mev$.
 Additionally, the region
 $\epsilon^2 <  5\times 10^{-7}$
 is excluded for   $m(A^{\prime})< 10.2\gev$,
 along with about half of the remaining few-loop 
region below the dimuon threshold. 
Many ideas have been proposed to further explore
the [$m(A^{\prime}),\epsilon^2$] 
parameter space 
%\cite{}[39–51], 
including an inclusive search for
$\decay{A^{\prime}}{\mu^-\mu^+}$ decays with the 
LHCb experiment,
 which is predicted to provide sensitivity to large regions of otherwise 
inaccessible parameter space using 
data to be collected during Run 3 of the LHC (in the years 2021 - 2024). 
%\cite{} [52].
A dark photon produced in proton-proton collisions via $\gamma^*–A^{\prime}$~mixing 
inherits the production mechanisms of an off-shell photon with
$m(\gamma^\ast)-m(A^{\prime})$; 
therefore, both the production and decay kinematics of the 
$\decay{A^{\prime}}{\mu^+\mu^-}$
and $\decay{\gamma^\ast}{\mu^+\mu^-}$ 
processes are identical.

LHCb performed searches for both prompt-like and long-lived dark photons \cite{DM-photon}
produced in pp collisions at a center-of-mass energy of 13~TeV, using 
$\decay{A^{\prime}}{\mu^+\mu^-}$
 decays and a data sample corresponding to an integrated luminosity of
1.6\invfb collected with the LHCb detector in 2016. 
The prompt-like $A^{\prime}$~search is 
performed from near the dimuon threshold up to 70~GeV, above which
the  $m(\mu^+\mu^-)$ 
spectrum is dominated by the \Z boson.
The long-lived $A^{\prime}$~search is restricted 
to the mass range
$214\leq m(A^{\prime})\leq 350\mev$,
where the data sample 
potentially provides sensitivity.


The prompt-like $A^{\prime}$~search is based on a data sample where all online-
reconstructed particles are stored, but most lower-level information is 
discarded, greatly reducing the event size. 
This data-storage strategy, made possible by advances in the LHCb data taking 
scheme introduced in 2015 
%\cite{}[59,60], 
permits the recording of all events that 
contain a prompt-like dimuon candidate without placing any requirements
on  $m(\mu^+\mu^-)$. 
Three main types of background contribute to the prompt-like $A^{\prime}$~search:
prompt $\decay{\gamma^\ast}{\mu^+\mu^-}$ 
production, which is irreducible; resonant decays to $\mu^+\mu^-$, whose mass 
peak regions are avoided in the search; and various types of misreconstruction.
 The misreconstruction background consists of three dominant contributions: 
double misidentification of prompt hadrons as muons, hh; a misidentified prompt
 hadron combined with a muon produced in a decay of a hadron containing a 
heavy-flavor quark, Q, where the muon is misreconstructed as prompt-like, 
h$\mu$Q; and the misreconstruction of two muons produced in Q-hadron decays, 
$\mu Q\mu Q$. 
These backgrounds are highly suppressed by the stringent muon-identification 
and prompt-like requirements applied in the trigger; however, in the region 
[m($\phi$),m($\Upsilon$)], the misreconstructed backgrounds overwhelm the 
signal-like 
$\decay{\gamma^\ast}{\mu^+\mu^-}$ 
contribution.
For masses below (above) the $\phi$ meson mass, dark photons are expected to be
 predominantly produced in meson-decay (Drell-Yan) processes in pp collisions 
at LHCb. 
A well-known signature of Drell-Yan production is dimuons that are largely 
isolated, and a high-mass dark photon would inherit this property. 
The signal sensitivity is enhanced by applying a jet-based isolation requirement
for $m(A^{\prime})>m(\phi)$,
which improves the sensitivity by up to a factor of two 
at low masses and by $O(10\%)$ for  $m(A^{\prime})\ge10\gev$. 
Jet reconstruction is performed by clustering charged and neutral particle-flow
 candidates 
%\cite{} [62] 
using the anti-kT clustering algorithm 
%\cite{}[63] 
with R = 0.5 as implemented in FastJet 
%\cite{}[64]. 
Muons with p$_T(\mu)/p_T$(jet) $<$ 0.7 are rejected, where the contribution to 
p$_T$(jet) from the other muon is excluded if both muons are 
clustered in the same jet, as this is found to provide nearly optimal 
sensitivity for all $ m(A^{\prime})>m(\phi)$. 
Figure 1 shows the resulting prompt-like
 $m(\mu^+\mu^-)$
 spectrum using $\Delta$ m bins that are 
$\sigma [m(\mu^+\mu^-)]/2$ 
wide, where 
$\sigma [m(\mu^+\mu^-)]/2$ 
is the mass resolution which varies from about 0.7\mev near threshold
to 0.7\gev at $m(\mu^+\mu^-) = 70\gev$.


For the long-lived dark photon search, the stringent criteria applied in the 
trigger make contamination from prompt muon candidates negligible. 
The dominant background contributions to the long-lived $A^{\prime}$~search are as 
follows: photon conversions to $\mu^+\mu^-$ in the silicon-strip vertex detector 
(the VELO) that surrounds the $pp$ interaction region 
%\cite{} [69]
; $b$-hadron decays 
where two muons are produced in the decay chain (a characteristic signature of muons produced in $b$-hadron decays is the 
presence of additional displaced tracks); and the low-mass tail from 
$K_S^0 \rightarrow \pi^+\pi^-$ 
decays, where both pions are misidentified as muons.
 Additional sources of background are negligible, e.g. kaon and hyperon decays,
 and Q-hadron decays producing a muon and a hadron that is misidentified as a
 muon.

Photon conversions in the VELO dominate the long-lived data sample at low masses. 
A high-precision three-dimensional material map was produced from a data sample
 of secondary hadronic interactions. 
Using this material map, along with properties of the  $\decay{A^{\prime}}{\mu^+\mu^-}$
 decay vertex and muon tracks, a $p$-value is assigned to
 the photon-conversion hypothesis for each long-lived  $\decay{A^{\prime}}{\mu^+\mu^-}$ candidate.

In these searches, no evidence for a signal is found, and 90\% CL exclusion regions are set
on the $\gamma-A^{\prime}$~kinetic-mixing strength. 
The constraints placed on prompt-like dark photons are the most stringent to 
date for the mass range   $10.6\leq m(A^{\prime})\leq 70\gev$,
and are comparable to the best existing limits for  $m(A^{\prime})\leq0.5\gev$. 
The search for long-lived dark photons is the first to achieve sensitivity 
using a displaced-vertex signature.
These results demonstrate the unique sensitivity of the LHCb experiment to dark
 photons, even using a data sample collected with a trigger that is inefficient
 for low-mass $\decay{A^{\prime}}{\mu^+ \mu^-}$ decays. 
Using knowledge gained from this analysis, the
 software-trigger efficiency for low-mass dark photons has been significantly 
improved for 2017 data taking. 
Looking forward to Run 3, the planned increase in luminosity and removal of the
 hardware- trigger stage should increase the number of expected
 $\decay{A^{\prime}}{\mu^+ \mu^-}$ decays in the low-mass region by a factor of 
$O(100–-1000)$ compared to the 2016 data sample.


==> giova-symbols-def.tex <==

%%% Alternate and additional macros for charmed baryons
\def\Lcp          {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcm          {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Lcpm         {{\ensuremath{\LorLbar{}^{\pm}_\cquark}}\xspace}
\def\Xicp         {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicm         {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Xicpm        {{\ensuremath{\XiOrXibar{}_\cquark^{\pm}}}\xspace}
\def\Xiczbar      {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xiczorbar    {{\ensuremath{\XiOrXibar{}_\cquark^0}}\xspace}
\def\Sigmacpp     {{\ensuremath{\Sigmares^{++}_\cquark}}\xspace}
\def\Sigmacmm     {{\ensuremath{\Sigmaresbar{}^{--}_\cquark}}\xspace}
\def\Sigmacpmpm   {{\ensuremath{\SigmaOrSigmabar{}^{\pm\pm}_\cquark}}\xspace}
\def\Sigmacp      {{\ensuremath{\Sigmares^{+}_\cquark}}\xspace}
\def\Sigmacm      {{\ensuremath{\Sigmaresbar{}^{-}_\cquark}}\xspace}
\def\Sigmacpm     {{\ensuremath{\SigmaOrSigmabar{}^{\pm}_\cquark}}\xspace}
\def\Sigmacz      {{\ensuremath{\Sigmares^{0}_\cquark}}\xspace}
\def\Sigmaczbar   {{\ensuremath{\Sigmaresbar{}^{0}_\cquark}}\xspace}
\def\Sigmaczorbar {{\ensuremath{\SigmaOrSigmabar{}^{0}_\cquark}}\xspace}
\def\Xiccbare     {{\ensuremath{\Xires_{\cquark\cquark}}}\xspace}
\def\Xiccpp       {{\ensuremath{\Xires^{++}_{\cquark\cquark}}}\xspace}
\def\Xiccmm       {{\ensuremath{\Xiresbar{}^{--}_{\cquark\cquark}}}\xspace}
\def\Xiccpmpm     {{\ensuremath{\XiOrXibar{}^{\pm\pm}_{\cquark\cquark}}}\xspace}
\def\Xiccp        {{\ensuremath{\Xires^{+}_{\cquark\cquark}}}\xspace}
\def\Xiccm        {{\ensuremath{\Xiresbar{}^{-}_{\cquark\cquark}}}\xspace}
\def\Xiccpm       {{\ensuremath{\XiOrXibar{}^{\pm}_{\cquark\cquark}}}\xspace}
\def\Omegaccp     {{\ensuremath{\Omegares^{+}_{\cquark\cquark}}}\xspace}
\def\Omegaccm     {{\ensuremath{\Omegaresbar{}^{-}_{\cquark\cquark}}}\xspace}
\def\Omegaccpm    {{\ensuremath{\OmegaOrOmegabar{}^{\pm}_{\cquark\cquark}}}\xspace}


\def\Xibcbare     {{\ensuremath{\Xires_{\bquark\cquark}}}\xspace}
\def\Xibbbare     {{\ensuremath{\Xires_{\bquark\bquark}}}\xspace}
\def\bbbar{b\overline{b}}

==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script python listsymbols.py

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash belletwo} & \belletwo & \texttt{\textbackslash besiii} & \besiii & \texttt{\textbackslash cleo} & \cleo \\
\texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern & \texttt{\textbackslash lhc} & \lhc \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron & \texttt{\textbackslash bfactories} & \bfactories \\
\texttt{\textbackslash bfactory} & \bfactory & \texttt{\textbackslash upgradeone} & \upgradeone & \texttt{\textbackslash upgradetwo} & \upgradetwo \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash emp} & \emp & \texttt{\textbackslash epem} & \epem \\
\texttt{\textbackslash muon} & \muon & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mupm} & \mupm & \texttt{\textbackslash mump} & \mump & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash taupm} & \taupm & \texttt{\textbackslash taump} & \taump & \texttt{\textbackslash tautau} & \tautau \\
\texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm & \texttt{\textbackslash ellp} & \ellp \\
\texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu & \texttt{\textbackslash neub} & \neub \\
\texttt{\textbackslash neue} & \neue & \texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neum} & \neum \\
\texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neut} & \neut & \texttt{\textbackslash neutb} & \neutb \\
\texttt{\textbackslash neul} & \neul & \texttt{\textbackslash neulb} & \neulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim & \texttt{\textbackslash pipm} & \pipm \\
\texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson & \texttt{\textbackslash rhoz} & \rhoz \\
\texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom & \texttt{\textbackslash rhopm} & \rhopm \\
\texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kbar} & \Kbar \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash Vzero} & \Vzero & \texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz \\
\texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb \\
\texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm \\
\texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash KorKbarz} & \KorKbarz & \texttt{\textbackslash etaz} & \etaz \\
\texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz & \texttt{\textbackslash omegaz} & \omegaz \\
\end{tabular*}

\subsubsection{Charmed mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Dbar} & \Dbar & \texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db \\
\texttt{\textbackslash DorDbar} & \DorDbar & \texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb \\
\texttt{\textbackslash Dp} & \Dp & \texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm \\
\texttt{\textbackslash Dmp} & \Dmp & \texttt{\textbackslash DpDm} & \DpDm & \texttt{\textbackslash Dstar} & \Dstar \\
\texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb \\
\texttt{\textbackslash theDstarz} & \theDstarz & \texttt{\textbackslash theDstarzb} & \theDstarzb & \texttt{\textbackslash Dstarp} & \Dstarp \\
\texttt{\textbackslash Dstarm} & \Dstarm & \texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp \\
\texttt{\textbackslash theDstarp} & \theDstarp & \texttt{\textbackslash theDstarm} & \theDstarm & \texttt{\textbackslash theDstarpm} & \theDstarpm \\
\texttt{\textbackslash theDstarmp} & \theDstarmp & \texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp \\
\texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dsmp} & \Dsmp \\
\texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp & \texttt{\textbackslash Dssm} & \Dssm \\
\texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp &  \\
\end{tabular*}

\subsubsection{Beauty mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash BdorBdbar} & \BdorBdbar \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash BsorBsbar} & \BsorBsbar \\
\texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm \\
\texttt{\textbackslash Bcpm} & \Bcpm & \texttt{\textbackslash Bds} & \Bds & \texttt{\textbackslash Bdsb} & \Bdsb \\
\texttt{\textbackslash BdorBs} & \BdorBs & \texttt{\textbackslash BdorBsbar} & \BdorBsbar &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chic} & \chic & \texttt{\textbackslash chiczero} & \chiczero \\
\texttt{\textbackslash chicone} & \chicone & \texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash chicJ} & \chicJ \\
\texttt{\textbackslash Upsilonres} & \Upsilonres & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chib} & \chib & \texttt{\textbackslash chibzero} & \chibzero & \texttt{\textbackslash chibone} & \chibone \\
\texttt{\textbackslash chibtwo} & \chibtwo & \texttt{\textbackslash chibJ} & \chibJ & \texttt{\textbackslash theX} & \theX \\
\end{tabular*}

\subsubsection{Light Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Lz} & \Lz & \texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar \\
\texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares \\
\texttt{\textbackslash Sigmaz} & \Sigmaz & \texttt{\textbackslash Sigmap} & \Sigmap & \texttt{\textbackslash Sigmam} & \Sigmam \\
\texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Sigmabarz} & \Sigmabarz & \texttt{\textbackslash Sigmabarp} & \Sigmabarp \\
\texttt{\textbackslash Sigmabarm} & \Sigmabarm & \texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiz} & \Xiz \\
\texttt{\textbackslash Xim} & \Xim & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Xibarz} & \Xibarz \\
\texttt{\textbackslash Xibarp} & \Xibarp & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Omegam} & \Omegam & \texttt{\textbackslash Omegabarp} & \Omegabarp &  \\
\end{tabular*}

\subsubsection{Charmed Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xic} & \Xic \\
\texttt{\textbackslash Xicz} & \Xicz & \texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar \\
\texttt{\textbackslash Xicbarz} & \Xicbarz & \texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac \\
\texttt{\textbackslash Omegacbar} & \Omegacbar & \texttt{\textbackslash Xicc} & \Xicc & \texttt{\textbackslash Xiccbar} & \Xiccbar \\
\texttt{\textbackslash Xiccp} & \Xiccp & \texttt{\textbackslash Xiccpp} & \Xiccpp & \texttt{\textbackslash Xiccbarm} & \Xiccbarm \\
\texttt{\textbackslash Xiccbarmm} & \Xiccbarmm & \texttt{\textbackslash Omegacc} & \Omegacc & \texttt{\textbackslash Omegaccbar} & \Omegaccbar \\
\texttt{\textbackslash Omegaccc} & \Omegaccc & \texttt{\textbackslash Omegacccbar} & \Omegacccbar &  \\
\end{tabular*}

\subsubsection{Beauty Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Sigmab} & \Sigmab \\
\texttt{\textbackslash Sigmabp} & \Sigmabp & \texttt{\textbackslash Sigmabz} & \Sigmabz & \texttt{\textbackslash Sigmabm} & \Sigmabm \\
\texttt{\textbackslash Sigmabpm} & \Sigmabpm & \texttt{\textbackslash Sigmabbar} & \Sigmabbar & \texttt{\textbackslash Sigmabbarp} & \Sigmabbarp \\
\texttt{\textbackslash Sigmabbarz} & \Sigmabbarz & \texttt{\textbackslash Sigmabbarm} & \Sigmabbarm & \texttt{\textbackslash Sigmabbarpm} & \Sigmabbarpm \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BR} & \BR & \texttt{\textbackslash BRvis} & \BRvis \\
\texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to &  \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, \boldmath \CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash T} & \T & \texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar \\
\texttt{\textbackslash Vud} & \Vud & \texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd \\
\texttt{\textbackslash Vus} & \Vus & \texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts \\
\texttt{\textbackslash Vub} & \Vub & \texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb \\
\texttt{\textbackslash Vuds} & \Vuds & \texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds \\
\texttt{\textbackslash Vuss} & \Vuss & \texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss \\
\texttt{\textbackslash Vubs} & \Vubs & \texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\texttt{\textbackslash Cpipi} & \Cpipi & \texttt{\textbackslash Spipi} & \Spipi & \texttt{\textbackslash CKK} & \CKK \\
\texttt{\textbackslash SKK} & \SKK & \texttt{\textbackslash ADGKK} & \ADGKK &  \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash Bsee} & \Bsee & \texttt{\textbackslash Bdee} & \Bdee \\
\texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk &  \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units (these macros add a small space in front)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}   } & \unit{kg}    &  \\
\end{tabular*}

\subsubsection{Energy and momentum }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevgev} & \gevgev \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevc} & \gevc & \texttt{\textbackslash mevcc} & \mevcc \\
\texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcc} & \gevgevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\end{tabular*}

\subsubsection{Distance and area (these macros add a small space)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst & \texttt{\textbackslash lumi} & \lumi \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash sqsnn} & \sqsnn \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash ptsq} & \ptsq & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash murad} & \murad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn & \texttt{\textbackslash git} & \git & \texttt{\textbackslash latex} & \latex \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbit} & \kbit & \texttt{\textbackslash kbps} & \kbps & \texttt{\textbackslash kbytes} & \kbytes \\
\texttt{\textbackslash kbyps} & \kbyps & \texttt{\textbackslash mbit} & \mbit & \texttt{\textbackslash mbps} & \mbps \\
\texttt{\textbackslash mbytes} & \mbytes & \texttt{\textbackslash mbyps} & \mbyps & \texttt{\textbackslash gbit} & \gbit \\
\texttt{\textbackslash gbps} & \gbps & \texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbyps} & \gbyps \\
\texttt{\textbackslash tbit} & \tbit & \texttt{\textbackslash tbps} & \tbps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbyps} & \tbyps & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}

\subsubsection{Helpful to align numbers in tables}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash phz} & \phz &  \\
\end{tabular*}



==> preamble1.tex <==
% THis file contains all the default packages and modifications for
% LHCb formatting

%% %%%%%%%%%%%%%%%%%%
%%  Page formatting
%% %%%%%%%%%%%%%%%%%%

% Allow the page size to vary a bit ...
\raggedbottom
% To avoid Latex to be too fussy with line breaking ...
\sloppy

%% %%%%%%%%%%%%%%%%%%%%%%%
%% Packages to be used
%% %%%%%%%%%%%%%%%%%%%%%%% 
%% \usepackage{microtype}
%% \usepackage{lineno}  % for line numbering during review
%%%%% \usepackage{xspace} % To avoid problems with missing or double spaces after
                    % predefined symbold


%% Graphics
\usepackage{graphicx}  % to include figures (can also use other packages)
\usepackage{color}
\usepackage{colortbl}
\graphicspath{{./figs/}} % Make Latex search fig subdir for figures

%% Math
\usepackage{amsmath} % Adds a large collection of math symbols
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{upgreek} % Adds in support for greek letters in roman typeset

%% fix to allow peaceful coexistence of line numbering and
%% mathematical objects
%% http://www.latex-community.org/forum/viewtopic.php?f=5&t=163
%%
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
\expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
\expandafter\let\csname oldend#1\expandafter\endcsname\csname
end#1\endcsname
 \renewenvironment{#1}%
   {\linenomath\csname old#1\endcsname}%
   {\csname oldend#1\endcsname\endlinenomath}%
}
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}%
}
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}

\usepackage{ifthenx} 
\newboolean{uprightparticles}
\setboolean{uprightparticles}{true} %Set true for upright particle symbols

% Get hyperlinks to captions and in references.
% These do not work with revtex. Use "hypertext" as class option instead.
\usepackage{hyperref}    % Hyperlinks in references
\usepackage[all]{hypcap} % Internal hyperlinks to floats.

%%%%%%%%%%% \input{lhcb-symbols-def} % Add in the predefined LHCb symbols

% Make this the last packages you include before the \begin{document}
%%% these two packages not working at the moment 

%%% \usepackage{cite} % Allows for ranges in citations
%%% \usepackage{mciteplus}

